Federated K-means Clustering

Federated learning is a technique that enables the use of distributed datasets for machine learning purposes without requiring data to be pooled, thereby better preserving privacy and ownership of the data. While supervised FL research has grown substantially over the last years, unsupervised FL methods remain scarce. This work introduces an algorithm which implements K-means clustering in a federated manner, addressing the challenges of varying number of clusters between centers, as well as convergence on less separable datasets.

==> sections/related_work.tex <==
\section{Background}
This work combines the K-means clustering algorithm and the federated learning paradigm. In this section, both these concepts will be discussed in more detail.

\subsection{K-means clustering}
The objective of a clustering algorithm is to partition a given dataset into several subsets with similar features. The K-means clustering algorithm does so by trying to minimize the so-called within cluster sum-of-squares criterion:
\begin{equation} \label{eq:inert}
    F_{km} = \sum_{j = 0}^m \min_{\mu_k \in C}(||X_{j,k} - \mu_k||^2)
\end{equation}
with $m$ the amount of samples, $\mu_k$ the cluster mean of cluster $k$, $C$ the set of all cluster means and $X_{j,k}$ being data point $j$ assigned to cluster $k$. The procedure in which the k-means algorithm tries to minimize equation \ref{eq:inert} consists of two steps. First, all data points get assigned to the cluster mean according to the lowest euclidean distance. Then, the mean value from all points assigned to a certain cluster is calculated. This is done for every cluster, creating a new set of means to start the next round with. This process is repeated until the change within these means is smaller than a certain threshold (and the algorithm has reached convergence) (\cite{KMeans}).
\subsection {Kmeans++}
One of the drawbacks of classical K-means clustering is that its initialization is sampled uniformly from the underlying data. This means that having initial cluster means that all come from the same cluster is as probable as having initial cluster means spread across all clusters. Although the K-means algorithm itself can somewhat compensate for this, it still leads to large variability in performance. \cite{KMeans++} developed an initialization method for K-Means to combat this high variability, called KMeans++. Instead of sampling K cluster means from the data with uniform probability, datapoints get weighted based on their distance to the closest already mean that is already chosen, with larger distances giving larger weights. This results in (on average) initializations that are more distributed over the space, and prevents (on average) initial cluster means from starting very close to each other, decreaseing K-means performance.




%\subsection{Federated learning} \label{sec:flback}
%The term Federated Learning (FL) was first coined in 2015 by Google \cite{fedAvg} as they were looking into ways of using smartphone text data for their natural language processing models, without having to download the data. The result was a paradigm shift in which the model moves to the data instead of the other way around. %In FL, there is a notion of a central server (without any data), which is connected to a set of local users (clients with data). The server is controlled by someone who wants to train a machine learning model, while the clients are devices owning a certain amount of data. First, the server sends out a certain machine learning model to (a subset of) clients, with weights randomly initialized. Then, clients train the received model for one or more epochs on their local data. These trained models are sent back to the server. The server aggregates the models, before sending them out to the clients again, and the cycle continues. The key idea is that by aggregating models from multiple clients into a single model, the resulting model is better than one of its parts. 
%The most widely used algorithm for aggregating these models is the one introduced by Google in 2015, called "federated averaging" \cite{fedAvg}. In federated averaging, model parameters are aggregated by taking the average for all model parameters, weighted by the sample size of the respective client. Once converged, the resulting model usually gives comparable results compared with a model trained on all data pooled together, while the server has not had access to a single sample of data \cite{FLbench1} \cite{FLbench2}.


